Reinforcement Learning of Adaptive Acquisition Policies for Inverse Problems

A promising way to mitigate the expensive process of obtaining a high-dimensional signal is to acquire a limited number of low-dimensional measurements and solve an under-determined inverse problem by utilizing the structural prior about the signal. In this paper, we focus on adaptive acquisition schemes to save further the number of measurements. To this end, we propose a reinforcement learning-based approach that sequentially collects measurements to better recover the underlying signal by acquiring fewer measurements. Our approach applies to general inverse problems with continuous action spaces and jointly learns the recovery algorithm. Using insights obtained from theoretical analysis, we also provide a probabilistic design for our methods using variational formulation. We evaluate our approach on multiple datasets and with two measurement spaces (Gaussian, Radon). Our results confirm the benefits of adaptive strategies in low-acquisition horizon settings.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections/topmatter.tex <==
\title{Variation Reinforcement Learning of Adaptive Acquisition Policies for Inverse Problems}

\author{....\\
Qualcomm AI Research \\
Qualcomm Technologies Netherlands B.V. \\
\texttt{\{....\}@qti.qualcomm.com} \\
}



==> sections_workshop/1_introduction.tex <==

\section{Introduction}
Compressed sensing aims at solving underdetermined linear inverse problems by leveraging the structure of the underlying signal of interest \citep{tibshirani1996regression,candes_stable_2006,donoho_compressed_2006}. Although the initial theory was focused on sparsity, other notions of structure have been considered too, for instance, in \citet{tang_compressed_2013}. Compressed sensing theory provides a hard constraint on the number of required measurements for signal recovery. Reducing the number of measurements is crucial when they are costly, for example, due to resource constraints or patient comfort in imaging tasks, and there has been a line of works exploring adaptive measurements to achieve this goal (see related works section). These works have been mainly focused on medical imaging applications like MRI where the space of measurements is a discrete space (see for example \citet{bakker2020experimental} and references therein). In this work, we aim to design a generic framework to solve adaptive recovery problems by simultaneously learning a measurement policy network and a recovery algorithm, while working with either continuous or discrete measurement spaces.
% In this work, we pursue two goals. First, we aim to design a generic framework to solve adaptive recovery problems by simultaneously learning a measurement policy network and a recovery algorithm. 
% The proposed framework works for continuous measurement spaces, where each measurement is chosen from a continuous space of actions. 
We stress that our method only needs to learn the measurement \textit{actions} and the recovery network. Thereby, our model can potentially be agnostic to the exact measurement model, making it a suitable candidate for non-linear settings. \textbf{Contributions.} \textbf{1)} We introduce a framework for adaptive sensing with arbitrary sensing operations that can naturally work in both continuous and discrete spaces. 
% In addition, our method can potentially be used with non-linear measurements, and can recover non-sparse signals, which are common constraints in Compressed Sensing literature.
\textbf{2)} We propose a novel training procedure for end-to-end learning of both reconstruction and acquisition strategies, which combines supervised learning of the signal to recover and reinforcement learning on latent space for optimal measurement selection.
% \textcolor{blue}{\sout{\textbf{4)} By reconsidering the existing theoretical work based on Gelfand width analysis (Cohen et al, 2009), we argue that the gain of adaptivity can show itself in average case error analysis and by considering adaptation as a  probabilistic procedure as done in our variational formulation.}}
% \arash{can you check this?}

% We would like to remark that our method only need to learn actions as measurement operation and a recovery network. Thereby, our model can potentially be agnositc to the exact measurement model making it a suitable candidate for non-linear settings. 
% , and can recover non-sparse signals, which are common constraints in Compressed Sensing literature.

==> sections_workshop/2_related_work.tex <==
\section{Related Work} \label{sec:related_works}
%%%%%%%%%%%%%%%%%%%%%
\subsection{Adaptive acquisition with Reinforcement Learning}
% I prefer to comment it
% \citet{Bora2017-as} introduce leveraging deep generative models for Compressed Sensing (CS) problems, which has since been extended in other works \citet{kuzina2022equivariant}. 
% The use of deep learning in Compressed Sensing (CS) has been introduced in \citet{Bora2017-as} and successfully used in works such as \citet{kuzina2022equivariant}, (\gian{TODO, more?}).

The question of adaptive compressed sensing has been approached from a  theoretical perspective in \citet{cohen_compressed_2009,foucart_gelfand_2010} (see \citet{foucart_mathematical_2013} for a concise and detailed overview of arguments based on Gelfand width). There are other works discussing various methods and theoretical analysis for the adaptive sensing \citep{malloy_near-optimal_2014,castro_adaptive_2014,castro_adaptive_2015,davenport_constrained_2016,braun_info-greedy_2015}. These works consider in general noisy setting, while we are focused on noiseless setting here. Their approach is classical and not data-driven.
In this work, we focus on Gelfand width-based analysis and review the subtleties of this argument in App. \ref{app:gelfand_bounds} and generalize some of the existing results. 
% There is a theoretical argument supporting that the adaptive acquisition does not help the reconstruction. see Chapter 10 of \citet{foucart_mathematical_2013} for a concise and detailed overview of arguments based on Gelfand width (as well as \citet{foucart_gelfand_2010}), and \citet{malloy_near-optimal_2014,castro_adaptive_2014,castro_adaptive_2015,davenport_constrained_2016,braun_info-greedy_2015} for other variants of the argument. We review the subtleties of this argument in \ref{app:gelfand_bounds} and generalize some of the existing results. 
Complementing traditional compressed sensing approaches which focus on solving the \textit{reconstruction} problem, we consider adaptive sensing approaches \citep{bakker2020experimental, pineda2020active, jin2019self, bakker2022learning, Ramanarayanan_2023_ICCV} where \textit{acquiring} measurements are treated as a sequential decision-making problem.
While our approach is closely related to the latter line of adaptive sensing techniques, we present a more general approach that is suitable beyond MRI scenarios, e.g., capable of dealing with both continuous and discrete sensing matrices and observations.
More importantly, we tackle both reconstruction and acquisition problems simultaneously thereby contrasting the two-stage training procedure, in which a model is first trained for reconstruction and subsequently for acquisition.
While the authors in \citet{yin2021end} also tackle these problems simultaneously, their approach trains the whole system in a supervised manner with short acquisition horizons (4 steps in their experiments).
To the best of our knowledge, we are the first to introduce an end-to-end training of reconstruction and acquisition models for active sensing with reinforcement learning.
% Compressed sensing differs from Adaptive sensing, or Adaptive acquisition, as in CS all the measurements are available at the same time and collected at random, while in Adaptive Acquisition, measurements are collected sequentially based on some strategy.
% Reinforcement Learning has been previously used to learn optimal adaptive acquisition strategies, in works such as \citet{bakker2020experimental, pineda2020active, jin2019self}. 
% Our approach is closely related to these works, but we do not restrict ourselves to the application to MRI reconstruction problem, and we propose a framework that can deal with a variety of compressed sensing scenarios, with both continuous and discrete sensing matrix and observations. All the aforementioned methods use a two-stage training procedure, in which they first train a reconstruction network and then an acquisition network. The method introduced in \citet{yin2021end} proposes instead to train both reconstruction network and acquisition network in an end-to-end fashion, showing superior results compared to training first reconstruction and then policy separately. However, such method trains the whole system with supervised learning, and uses short acquisition horizons (4 steps in their experiments). To the best of our knowledge, we are the first to introduce and end-to-end training of reconstruction and acquisition framework for active sensing with reinforcement learning.
% (\gian{do we need to reference experimental design? Also description a bit weak, please double check})
% Adaptive acquisition shares many similarities with methods for Experimental Design, such as \citet{foster2021deep, blau2022optimizing}, where the goal is to maximise the expected information gain of the experiments.
Our method also extends the work of \citet{zintgraf2019varibad}, which proposes a method to learn a belief distribution over unknown environments. 
While we use a similar architecture and training procedure, our work differs in its goal. The work \citet{zintgraf2019varibad}  performs meta-learning over the transition probability and reward function of unknown environments while we train our models to extract a belief distribution over the unknown state of a POMDP, similarly to \citet{igl2018deep, lee2020stochastic}.
In addition, the decoder in \citet{zintgraf2019varibad} is used to predict the future (and the past) of a Bayesian Augmented MDP, while for us, it is used as a reconstruction network, which is crucial to our end goal, namely to achieve a reconstructed signal faithful to the original signal $\vx$. 
% In App. \ref{app:gelfand_bounds}, we argue that adding this probabilistic component can be potentially helpful for getting gains of adaptive sensing.
% Finally, our method borrows many building blocks from \citet{zintgraf2019varibad}, which proposes a method to learn a belief distribution over unknown environments. We use a very similar architecture and training procedure, but our works differ in purpose. \citet{zintgraf2019varibad} is introduced to perform meta-learning over the transition probability and reward function of unknown environments, while we train our models to extract a belief distribution over the unknown state of a POMDP, similarly to \citet{igl2018deep, lee2020stochastic}. In addition, the decoder in \citet{zintgraf2019varibad} is used to predict the future (and the past) of a Bayesian Augmented MDP, while for us it is used as reconstruction network, which has a crucial role as our end goal is to achieve a reconstructed signal $\hat{x}$ as close as possible to the original signal $x$.
% There is a theoretical argument supporting that the adaptive acquisition does not help the reconstruction. see Chapter 10 of \citet{foucart_mathematical_2013} for a concise and detailed overview of arguments based on Gelfand width (as well as \citet{foucart_gelfand_2010}), and \citet{malloy_near-optimal_2014,castro_adaptive_2014,castro_adaptive_2015,davenport_constrained_2016,braun_info-greedy_2015} for other variants of the argument. We review the subtleties of this argument in \ref{app:gelfand_bounds} and generalize some of the existing results. 
% \tribhu{@GS: Let's drop this paragraph?}
% To summarize, the gain of adaptive acquisition disappears whenever...
%%%%%%%%%%%%%%%%%%%%%
\subsection{Latent Variable models and Deep RL}
The papers \citet{chung2015recurrent, gregor2018temporal} introduce variational methods for modeling temporal sequences, arguing that it is important to have a latent representation that can form a belief distribution representing a measure of uncertainty. We draw inspiration from these works to introduce a probabilistic interpretation of the latent space in our model.
Our architecture and training procedure are similar to the ones used in Reinforcement Learning on latent space methods \citep{khan2019latent, allshire2021laser, zhou2021plas}, Meta Reinforcement Learning \citep{wang2016learning, duan2016rl, zintgraf2019varibad} and Model-Based Reinforcement Learning \citep{hafner2019dream, hafner2020mastering}. In the context of POMDPs, works such as \citet{igl2018deep, hafner2019learning, lee2020stochastic} use Deep Variational Reinforcement Learning to learn a belief distribution over the hidden state, showing how explicitly modeling the uncertainty improves the performance of the agent. In our work, such belief distribution must be suitable for both the acquisition and reconstruction networks to select the follow-up action and reconstruct the unknown signal $\vx$.

==> sections_workshop/3_method.tex <==
\section{Methodology}
\label{sec:method}
As in compressed sensing, we consider underdetermined inverse problems, where the goal is to recover a high-dimensional \textit{signal} $\vx \in \R^N$ through low-dimensional \textit{observations} $\vy \in \R^T (T \ll N)$. 
Each observation $y_t = F(\va_t, \vx)$ is acquired through a projection operation parameterized as $\va_t$.
In a linear measurement setting, this amounts to $\vy = F(\mA, \vx) = \mA \vx$
where $\mA \in R^{T \times N}$ is referred to as the `sensing matrix', and is defined as $\mA = [\va_1, \va_2, \dots, \va_T]^\top$.
% and $\Psi \in R^{N \times N}$ as the `dictionary'.
% For simplicity, we refer to the product $\mA = \Phi \Psi$ as the sensing matrix which is a result of stacking $T$ projections $\va_t$.
We will explain specific types of $\mA$, $\vx$, $y$, and $F$ used in this work in section \ref{sec:datasets}.
The primary goal in the compressed sensing setup is to recover the signal $\vx$.
Note that this reconstruction is generally intractable as it amounts to solving an under-determined system of equations.
However, the reconstruction becomes possible if we assume a prior about the signal structure, for example, the assumption of sparsity or lying on the data manifold modeled by a deep generative model \citep{Bora2017-as}.
An auxiliary goal in compressed sensing is to reduce the number of measurements (i.e., the number of rows in $\mA$) with minimal impact on the recovery process.
This is especially critical when the measurement process is an expensive, time-consuming process, such as with medical MRI or CT scans.
Reducing the measurements can be achieved by designing a better measurement matrix $\mA$. The above two goals present an inherent trade-off: we can obtain better reconstructions at the price of collecting more expensive, time-consuming measurements.
In the next section, we present our technique that jointly addresses this trade-off. For an overview of the related work, the reader is referred to Appendix \ref{sec:related_works}. For a schematic representation of our method, see Appendix \ref{app:more_figures}.

\subsection{Adaptive Compressed Sensing}



\textbf{Framework.}
Central to our approach towards minimizing the number of measurements is exploiting adaptivity:
to sequentially construct the sensing matrix $\mA$ (composed of $T$ projection vectors $\va_t$) to enable better recovery of the underlying signal $\vx$.
Similar to \citet{bakker2020experimental}, we approach this sequential decision-making problem within a reinforcement learning framework. In the following, we use the terms active and adaptive strategies interchangeably, meaning strategies that select custom measurements depending on the specific input or signal.\\
\textbf{Adaptive Acquisition as a POMDP.} We define the adaptive acquisition as a Partially Observable Markov Decision Process (POMDP). A POMDP is defined by a tuple ($\gS$, $\gA$, $\gO$, $\gF$, $\gU$, $\gR)$.
Here, $\gS$ is the state space, 
$\gA$ the action space, 
$\gO$ the observation space,
$\gF: (\gS \times \gA) \rightarrow \gS$ is the transition distribution, 
$\gU: (\gS \times \gA) \rightarrow \gO$ is the observation distribution, and
$\gR: (\gS \times \gA) \rightarrow \R$ is the reward function for a state-action pair.
Over the next paragraphs, we take a closer look at each of these aspects of the problem of adaptive compressed sensing.\\
\textbf{Stationary State and Transition Distribution.}
We consider the signal $\vx$, which needs to be recovered as the stationary state of the system.
The agent cannot directly observe the state but rather senses and obtains low-dimensional observations $y_t$.
As a result of the stationary state, the transition distribution remains fixed, $\mathcal{F}(\vx_{t+1}\mid \vx_t, \va_t) = \delta(\vx_{t+1}-\vx_t)$, $\vx_0=\vx$, which means that $\vx_{t+1} \sim \delta(\vx_{t+1}-\vx)$, where $\delta$ is the Dirac distribution.\\
\textbf{Actions.}
Each action $\va_t$ corresponds to a particular projection operation, i.e., a row of the sensing matrix $\mA$.
Depending on the type of measurement used (more details in \ref{sec:datasets}), the actions can take different forms but generally are $N$-dim real-valued vectors.\\
\textbf{Observations and Observation Distribution.}
We denote as \textit{observation} $y_t$ the information received by the agent after performing a measurement $y_t = F(\va_t, \vx)$. 
This observation is drawn from observation distribution $y_t \sim \gU(y_{t} | \vx, \va_t)$.
Since the paper primarily studies reconstructing a time-invariant signal in a noiseless setting, the observation corresponds to a deterministic measurement $y_t = F(\va_t, \vx)$.\\
\textbf{Reward.}
After taking an action, the agent receives a reward according to the distribution $r_{t} \sim \mathcal{R}(r_{t}\mid \vx, \va_t)$. 
We define the reward at each time step as the improvement in reconstruction quality $d(.)$ between consecutive time steps: $r_{t} = d(\hat{\vx}_{t}, \vx) - d(\hat{\vx}_{t-1}, \vx)$ following a metric $d$. 
In our experiments, we use Structural Similarity Index Measure (SSIM) \citep{wang2004image} as $d(.)$. 
For $t=1$, the reward is simply $d(\hat{\vx}_{1}, \vx)$.

\subsection{Architectural components}
\label{sec:method_architecture}

Central to our approach are two models:
(a) a \textit{reconstruction} model that recovers the signal from low-dimension observations; and
(b) an \textit{acquisition} model (the agent) that adaptively constructs the sensing matrix for measurements.
We now look into these models in-depth.\\
\textbf{Reconstruction Model.}
The goal of the reconstruction model is to recover a signal $\hat{\vx}_t$ that faithfully represents the signal $\vx$ under measurement.
Such a recovery is challenging, given that the system is under-determined, i.e., we recover using $T$ measurements $\vy_{1:T}$ while the signal is $N$-dimensional ($N \gg T$).
To tackle this challenge, inspired by \citet{bakker2020experimental}, we use an autoencoder-style model to perform reconstruction but with one key difference:
the encoder is a Gated Recurrent Unit (GRU) \citep{cho2014properties} designed to deal with variably-sized sequences.
The autoencoder is defined by a (recurrent) encoder $g_\phi$ and a decoder $f_\phi$, both parameterized by $\phi$. 
At each time-step $t$, the encoder predicts the latent features $z_t$ from the trajectory of actions $\va_{1:t}$ and observations $\vy_{1:t}$, $\vz_t = g_\phi(\va_t, \vy_t, \vh_t)$, where $\vh_t$ is the hidden state of the GRU and summarizes the past inputs $a_{1:t-1}$ and $y_{1:t-1}$.
The decoder receives $\vz_t$ as input and outputs a reconstruction $\hat{\vx}_t$: $\hat{\vx}_t = f_\phi(\vz_t).$ The model is trained to minimize a loss $\mathcal{L}$ defined as the sum of the Mean Squared Error (MSE) between $x$ and $\hat{x}_t$ for each $t$, $\mathcal{L} = \frac{1}{T}\sum_{t=1}^{T} (\vx - \hat{\vx}_t)^2$.
As opposed to solely considering the MSE with the final reconstruction $\hat{\vx}_{T}$, our formulation presents certain benefits:
(a) it takes into account the scenario in which $\vx$ changes over time (e.g., when taking a measurement affects the true signal);
(b) it forces the model to have good reconstruction quality at each time step.\\
\textbf{Acquisition Model (Policy Network).}
The goal of the acquisition model is to predict a projection (the action) $\va_t$, such that the resulting observation $\vy_t = F(\va_t, \vx)$ is highly informative towards reconstructing the signal $\hat{\vx}_t$.
To achieve this goal, we design a policy to select the next action based on the history of measurements, observations, and reconstruction qualities.
Therefore, we condition the policy network on the encoder's latent representation $\vz_{t-1} = g_\phi(\va_{t-1}, \vy_{t-1}, \vh_{t-1})$, which is in parallel also used to aid reconstruction as we saw earlier. Therefore, the policy learns to select the next action $\va_{t+1}$ conditioned only on the latest latent representation, $\va_{t} \sim \pi_\theta(\va_{t} \mid \vz_{t-1})$
This differs from what is commonly done in Adaptive Sensing for MRI, where the policy is conditioned on the latest reconstruction $\hat{x}_t$ \citep{bakker2020experimental}.
Following this acquisition, we reconstruct the signal based on the latest observation to assign an instantaneous reward $r_{t}$. More details regarding the training of the policy network are reported in Appendix \ref{app:pg}.
\subsection{Training strategy and Baselines}
\label{sec:method_training}
In this section, we walk through our end-to-end approach where the reconstruction and adaptive acquisition model are jointly trained.
We begin discussing two baseline approaches and conclude with the end-to-end approach.\\
\textbf{Baseline 1: Random Acquisition and Reconstruction (\texttt{AE-R}).} In this baseline, we consider a random acquisition policy: each action taken is drawn agnostic to past actions, observations, and rewards. \\
\textbf{Baseline 2: Adaptive Acquisition with pre-trained Reconstruction (\texttt{AE-P}).} The second baseline consists of a pre-trained reconstruction model, trained with the same procedure used for the \texttt{AE-R} baseline. 
This strategy is similar to that proposed in \citet{bakker2020experimental}.
The policy selects a first measurement $\va_1$, which is used to obtain a first observation $y_1$. 
Then, for $t = 1,\dots,T$, we compute $\vz_t = g_\phi(\va_t, \vy_t, \vh_t)$ ($\vh_1$ is filled with zeros) and $\hat{\vx}_t=f_\phi(\vz_t)$. 
The policy selects the next action $\va_{t+1}$ based on $\vz_t$, and the procedure is repeated until the entire trajectory is collected. 
Finally, the policy is updated with Policy Gradient (see section \ref{app:pg}), while the reconstruction model is kept fixed.
The policy network is always trained on the same data used to pre-train the reconstruction network.\\
\textbf{End-to-End Adaptive Acquisition and Reconstruction (\texttt{AE-E2E}).} We proposed end-to-end training of both reconstruction and acquisition models. 
Unlike the previous \texttt{AE-P} strategy, the reconstruction model is now initialized with random parameters and is trained after each trajectory is collected by the policy. 
Inspired by \citet{zintgraf2019varibad}, we do not backpropagate gradients from the policy to the encoder, to avoid instabilities and the need for additional hyperparameters for the multi-task learning loss.

% We consider three different strategies to train reconstruction and acquisition models: 
% (a) Reconstruction with Random Acquisition (\texttt{AE-R}); 
% (b) Adaptive Acquisition with pretrained Reconstruction (\texttt{AE-P}); and 
% (c) End-to-end training of both Reconstruction and Acquisition (\texttt{AE-E2E}).

% \myparagraph{Reconstruction with Random Acquisition}
% This model is used as baseline, and consists in the reconstruction model used standalone, with a policy that outputs action at random, following some predefined probability distribution. Note that in this case there is no inherent concept of temporal sequences, as all the measurements are done in parallel and independently of each other, therefore removing the need for a recurrent encoder. However, to make the baseline comparable with other acquisition strategies in which there is a sequential acquisition, we decided to keep the same architectural components.

% \myparagraph{Adaptive Acquisition with pretrained Reconstruction}
% The second model consists of a pretrained reconstruction model, trained with the same procedure used for the AE-R baseline. This is the same procedure proposed in \citet{bakker2020experimental}. The policy selects a first measurement $a_1$, which is used to obtain a first observation $y_1$. Then, for $t = 1,\dots,T$, we compute $z_t = g_\phi(a_t, y_t, h_t)$ ($h_1$ is filled with zeros) and $\hat{x}_t=f_\phi(z_t)$. The policy selects the next action $a_{t+1}$ based on $z_t$, and the procedure is repeated until the whole trajectory is collected. Finally, the policy is updated with Policy Gradient (see section \ref{sec:method_architecture}), while the reconstruction model is kept fixed.
% The policy network is always trained on the same data used to pretrain the reconstruction network.

% \myparagraph{End-to-end training of both Reconstruction ad Acquisition}
% The last training strategy consists in training end-to-end both reconstruction and acquisition models. It is the same as the AE-P strategy, but the reconstruction model is initialized with random parameters and trained after each trajectory is collected by the policy. Inspired by \citet{zintgraf2019varibad}, we decide to not backpropagate gradients from the policy to the encoder, to avoid instabilities and the need for additional hyperparameters for the multi-task learning loss.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.45\textwidth]{images/detenc.pdf}
% \caption{End-to-end training of encoder, decoder and policy. The gradients from the policy are not backpropagated through to the encoder.}
% \label{fig:detenc}
% \end{figure}


% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.45\textwidth]{images/varenc.pdf}
% \caption{End-to-end variational training of encoder, decoder and policy. The gradients from the policy are not backpropagated through to the encoder.}
% \label{fig:varenc}
% \end{figure}


% \subsection{Introducing Bayesian Reasoning}

% \section{(Deprecated) Methodology}

% In this work, we consider the case of compressed sensing in which we have a sensing matrix $A$ and matrix of observations $y$, deriving from the source signal $x$ following some transformation $F$:
% \begin{align}
%     y = F(A,x)
% \end{align}
% In the adaptive sensing scenario, we want to adaptively and sequentially select and add rows to the sensing matrix $A$, to obtain new information regarding $x$ trough $y$, and keep adding measurements based on the quality of the reconstruction of $x$. It is therefore crucial to use methods that can handle varying size input, and a sensible choice is to use recurrent neural networks. We can in fact consider each row of $A$ and $y$ as a different time step, and train a recurrent unit to extract information from them while keeping memory of the past. Similarly to \citet{bakker2020experimental}, we propose here a method for training a reconstruction algorithm that is capable of recovering $x$ given $A$ and $y$, and then use a reinforcement learning algorithm to learn an optimal acquisition strategy given the pretrained reconstruction network.

% \subsection{Reconstruction and acquisition for active sensing}
% While the method proposed in \citet{bakker2020experimental} is limited to work with discrete measurements for images, we propose an extension that can be trained with arbitrary sensing matrices and observations, with either continuous or discrete values. We start by highlighting that the Vanilla Policy Gradient algorithm used in \citet{bakker2020experimental} can naturally deal with both continuous and discrete action spaces. We keep the autoencoder-like structure used in \citet{bakker2020experimental} for the reconstruction model, but change the encoder to be a GRU (TODO, cite GRUs). In this way, we can deal with sequences of measurements and observations of arbitrary length, and we can process them in an online fashion. We start by pre-training the autoencoder by sequentially feeding randomly sampled sensing matrix rows and the corresponding observations. We then proceed by training the policy. While \citet{bakker2020experimental} conditions the policy on the latest reconstructed signal, we decide instead to condition on the latest latent space representation of the autoencoder, since following the manifold hypotesis assumption, the latent space should contain all the necessary information of the reconstructed image in a much more compact representation \citet{pope2021intrinsic, fefferman2016testing, bengio2013representation}.
% \subsection{End-to-end reconstruction and acquisition}
% Methods such as \citet{yin2021end} propose instead to train both reconstruction network and policy network in an end-to-end fashion, showing superior results compared to training first reconstruction and then policy separately. However, such method trains the whole system in a supervised learning fashion, therefore treating the policy as a simple neural network. To the best of our knowledge, we are the first to introduce and end-to-end reconstruction and acquisition framework for active sensing with reinforcement learning (are we though? need to check recent literature). Our end-to-end system works in the following way: we first sample an initial measurement (or action) from the policy and compute the corresponding observation. We then feed these to the (recurrent) encoder, and obtain a latent representation of the state. The decoder will then use such representation to reconstruct the image, while the policy will use it to select the next measurement. We repeat this procedure until a predefined number of measurements is reached. To train the autoencoder, we use the sum of MSE from the reconstructions at each time step, while the policy uses as reward the difference in SSIM for the reconstruction between consecutive time steps. Inspired by \citet{zintgraf2019varibad}, we decide to not backpropagate gradients from the policy to the encoder, to avoid instabilities and the need for additional hyperparameters for the multi-task learning loss.
% \subsection{Bayesian reasoning and the importance of belief states}
% While the end-to-end training for reconstruction and acquisition presents appealing properties, it might also be affected by the weaknesses of simple autoencoder models, which tends to learn an unstructured latent space which can result in overfitting \citet{chung2015recurrent}. Furtermore, it might be beneficial for the policy to receive as input, in addition to the latent space, a measure of uncertainty about it, to represent how confident the encoder is about the signal $x$ after having seen a sequence of $t$ measurements $a_{1:t}$ and observations $y_{1:t}$. In fact, the policy might learn to select exploratory actions when the uncertainty is high, and select more exploitative actions as the uncertainty decreases. We therefore introduce a variational formulation for our model, inspired by \citet{zintgraf2019varibad}, to learn a belief representation of the latent space $b(z_t \mid a_{1:t}, y_{1:t})$, which is then used by the decoder, which will model the likelihood $p(x\mid z_t\sim b(z_t \mid a_{1:t}, y_{1:t}))$, and by the policy $\pi(a_{t+1} \mid b(z_t \mid a_{1:t}, y_{1:t}))$, which will select the next action based on the current belief. The lower bound derivation can be found in Appendix \ref{app: lower_bound}. The training procedure remains the same as for the deterministic end-to-end case, but now the encoder $g(y_t, a_t, h_t)$ parametrizes mean $\mu_g$ and standard deviation $\sigma_g$ of the posterior belief distribution $b(z_t \mid a_{1:t}, y_{1:t})$, the decoder will reconstruct $x$ given samples from the belief $z_t\sim b(z_t \mid a_{1:t}, y_{1:t})$, and the policy will instead receive the parameters of the belief distribution, so $\pi(a_{t+1}\mid \mu_g, \sigma_g)$.

% \subsection{Theoretical insight}

% In App. \ref{app:gelfand_bounds}, we consider the argument based on Gelfand width analysis against the gain of adaptive sensing. In the classical result, the focus has been on the worst-case error for deterministic recovery algorithms and adaptive schemes that rely only on the outcome of previous measurements and not on the intermediate reconstruction. We extend the existing results and show that a similar result can be obtained even if we extend the adaptive schemes to use previous reconstructions as input or fix the recovery algorithm. This means that we might not expect additional gain by using previous reconstructions. 
% We argue for two insights from the theory. First, the gain can show itself if we move away from worst-case error analysis. Second, we argue that the theory does not apply to a probabilistic adaptive scheme. This is a motivation behind using probabilistic formulations as presented above to get gains from adaptive sensing. 


==> sections_workshop/4_experiments.tex <==
\section{Experiments}\label{sec:experiments}
% In this section, we describe the experiments performed to evaluate the propose method. We first describe the datasets used, and then provide a comparison for the three methods introduced above, AE-R, AE-P and AE-E2E. Finally, we verify the effectiveness of the variational formulation introduced in section \ref{sec:method_bayes}. Additional experiments can be found in Appendix \ref{app:exp_ppo}, where we analyze a phenomenon observed in \citet{bakker2020experimental}, where greedy policies ($\gamma = 0$) seem to perform better than discounted ones. Note that we focus on continuous action spaces. Moreover, we report additional ablation studies and complementary results for some of the datasets in Appendix \ref{app:more_figures} and \ref{sec:abl_stuides}. 
% While our method can in principle deal with non-linear CS problems, we do not experiment with those in this work.

In this section, we describe the experiments performed to evaluate the proposed method. We first describe the datasets used, and then provide a comparison of the three methods introduced above, AE-R, AE-P, and AE-E2E.
While our method can in principle deal with non-linear CS problems, we do not experiment with those in this work. We provide a variational formulation for the autoencoder in Appendix \ref{sec:method_bayes}. We further refer the reader to Appendix \ref{app: experiments} for more experimental results, including experiments on the Low Dose CT Image and Projection Data\footnote{\url{https://www.aapm.org/grandchallenge/lowdosect/}} (MAYO) dataset \citep{moen2021low}.

\subsection{Datasets and Sensing Operations}
\label{sec:datasets}
% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-7mm}
% \centering
% \includegraphics[width=0.95\linewidth]{images/gauss.pdf}
% \caption{Example of Gaussian measurement, with random acquisition. Each element of $a_t$ is independently sampled from a standard Gaussian, and multiplied (dot product) with the signal $x$ to obtain the corresponding observation $y_t$.}
% \label{fig:gauss}
% \end{wrapfigure}
We test our algorithms for adaptive acquisition the handwritten digits dataset MNIST \citep{deng2012mnist}. We use two different sensing operations $F$, which we name as \textit{Gaussian} and \textit{Radon}.
The Gaussian transformation, denoted as $G$, consists in a matrix multiplication between a random Gaussian matrix $\mA$ and the flattened image $\vx$: 
% \begin{align}
$\vy = G(\mA,\vx) = \mA\vx$.
% \end{align}
The rows $\va_t$ of the sensing matrix have continuous entries $\in(-\infty, \infty)$, and same for $\vy$. For a vectorized image of size $N\times1$, the sensing matrix has size $T\times N$ (each row $\va_t$ is $1\times N$, with $T$ the total number of acquisitions, and $\vy$ is a vector of dimensions $1\times T$. In the adaptive acquisition scenario, the resulting $y_t=G(\va_t, \vx)$ is a scalar. Note that in compressed sensing, Gaussian measurements can achieve theoretical limits for non-adaptive sensing, and therefore represent the best non-adaptive sensing scheme.
% A visual example is provided in Figure \ref{fig:gauss}.
The Radon transform is commonly used to reconstruct images from CT scans, see \citet{beatty2012radon} for a detailed description.
The sensing matrix $\mA$ corresponds to a vector $1\times T$ of angles in radians, with each $a_t$ being a scalar $\in [-\pi, \pi]$. Assuming that $x$ is an image of dimensions $h\times w$, then the $\vy$ resulting from $R(\mA,\vx)$ is a matrix of dimensions $h\times T$.
In adaptive acquisition, $y_t = R(a_t, \vx)$ is a vector of dimensions $h\times 1$. 

\subsection{Random vs Adaptive Acquisitions}
\label{sec:exp_ae}
We compare the performance of AE-R, AE-P, and AE-E2E models introduced in section \ref{sec:method_training} on the MNIST dataset, for both Gaussian and Radon sensing operations. We experiment with different trajectory length, $T=20, 50, 100$ for Gaussian and $T=5, 10, 20$ for Radon. This choice is motivated by Radon measurements providing more information than Gaussians (a vector instead of a scalar).
The results are reported in table \ref{tab:random_vs_e2e_mainpaper}. We also report the reconstruction quality in SSIM after each acquisition step for models trained to optimize the whole trajectories, in Appendix \ref{app:full_mnist}.

\input{tables_iclr/mnist_random_vs_adaptive_mainpaper.tex}

From the results, we can see how AE-E2E outperforms the other methods in most cases. However, while in Radon longer trajectories lead to higher performance, that is not the case for Gaussian measurements, where increasing the number of measurements leads to worse performance. Note, however, that this is the case only for the adaptive strategies, while AE-R keeps improving performance the more we add measurements and observations. We conjecture that this behavior could be related to the high dimensionality of the action space for the policy with Gaussian measurements. However, the adaptive E2E model still performs better for trajectories of length $\sim 40$, which is more than is used in papers such as \citet{bakker2020experimental, yin2021end}.



==> sections_workshop/5_conclusion.tex <==
\section{Conclusion}
We introduce a novel framework for end-to-end training of reconstruction and acquisition in generic compressed sensing problems. We show how using adaptive acquisition strategies can improve over random measurements, especially for a limited number of acquisition steps.\\
\textbf{Future work.}
Our method does not outperform the random baseline in the cases of long acquisition horizons and high-dimensional action space. This is expected as random measurements are known to be theoretically optimal when a sufficiently long measurement horizon is available. Nonetheless, we propose some future directions to potentially improve upon our results.
A careful tuning of discount factor and other policy parameters can improve performances (see App. \ref{app:exp_ppo}).
For the case of Gaussian measurements, the dimensionality of the action space scales quadratically with the dimension of the images. Results suggest that this might be a major drawback, as the policy seems to find it difficult to select optimal actions in such a vast action space. Better ways to parametrize the probabilistic policy space could substantially improve the results, alongside more sophisticated policy learning strategies that can deal with such a complex search space.

==> sections_workshop/7_ablation_studies.tex <==
\subsection{Ablation Studies}\label{sec:abl_stuides}
The purpose of this section is to report results from ablation studies. We report results concerning the MNIST and MAYO datasets. According to the main paper, also in this section, we consider Gaussian and Radon measurements. As we already mentioned in~\autoref{sec:datasets}, we base our choice of Gaussian and Radon type of measurements on the following observation. In compressed sensing, Gaussian measurements can achieve theoretical limits for non-adaptive sensing and therefore represent the best non-adaptive sensing scheme. Instead, the Radon transform represents a common choice to reconstruct images from CT scans (see \citet{beatty2012radon} for a detailed description).
In~\autoref{tab:random_vs_e2e_mnist_abl} to~\autoref{tab:beta_vae_mayo_abl} we report results concerning models trained using the final reward only, i.e., we consider only the reconstruction error at the final state (after $T$ measurements). We rerun the simulations on the MNIST dataset multiple times. It is possible to notice how in~\autoref{tab:random_vs_e2e_mnist_abl} and~\autoref{tab:beat_vae_mnist_abl} the results are significantly worse than the cases in which reward is given at each time step, indicating that the increased sparsity in the reward distribution results to be more challenging for the policy, especially as the acquisition horizon increases. A different result can be seen in~\autoref{tab:random_vs_e2e_mayo_abl} and ~\autoref{tab:beta_vae_mayo_abl}, where the performances seem to improve with respect to the results in~\autoref{tab:mayo}, even though not always with increased number of acquisition. From these results, we can conclude that the two different kinds of rewards may be suited for different models and datasets and that both should be tested.


\input{tables_iclr/new_res_1}
\input{tables_iclr/new_res_2}
\input{tables_iclr/new_res_3}
\input{tables_iclr/new_res_4}
% \include{tables/NewResults}



==> sections_workshop/topmatter.tex <==
\title{Variation Reinforcement Learning of Adaptive Acquisition Policies for Inverse Problems}

\author{....\\
Qualcomm AI Research \\
Qualcomm Technologies Netherlands B.V. \\
\texttt{\{....\}@qti.qualcomm.com} \\
}



==> tables/NewResults.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean on the row signed as M, while we report the worst
    case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    \small
    \begin{tabularx}{\linewidth}{llcccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.505 \pm .018$ & $.641 \pm .014$ & $.726 \pm .011$ & $.658 \pm .014$ & $.664 \pm .014$ & $.757 \pm .011$ \\
         & \multirow{1}{*}{W}   & $-.028$ & $.064$ & $.132$ & $.074$ & $-.036$ & $.100$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.325 \pm .021$ & $.217 \pm .018$ & $.232 \pm .016$ & $.680 \pm .013$ & $.456 \pm .019$ & $.365 \pm .017$ \\
         & \multirow{1}{*}{W}   & $-.117$ & $-.153$ & $-.119$ & $.079$ & $-.120$ & $-.111$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & $.475 \pm .021$ & $.296 \pm .021$ & $.283 \pm .021$ & $.824 \pm .009$ & $.781 \pm .014$ & $.739 \pm .015$ \\
         & \multirow{1}{*}{W}   & $-.078$ & $-.162$ & $-.144$ & $.205$ & $.057$ & $.010$ \\
         \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mnist_abl}
    \end{center}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \small
    \begin{tabularx}{1.04\linewidth}{llcccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & $\beta$ & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.441 \pm .018$ & $.627 \pm .014$ & $.703 \pm .012$ & $.566 \pm .016$ & $.639 \pm .015$ & $.733 \pm .012$ \\
         & $.1$ & $.467 \pm .017$ & $.629 \pm .015$ & $.701 \pm .012$ & $.581 \pm .015$ & $.678 \pm .012$ & $.743 \pm .011$ \\
         & $.01$ & $.482 \pm .016$ & $.635 \pm .014$ & $.696 \pm .012$ & $.595 \pm .014$ & $.714 \pm .012$ & $.761 \pm .010$ \\
         & $.001$ & $.479 \pm .016$ & $.635 \pm .014$ & $.706 \pm .012$ & $.612 \pm .014$ & $.675 \pm .013$ & $.764 \pm .010$ \\
         \midrule
         
        \multirow{3}{*}{VAE-P} 
        & $1$ & $.335 \pm .019$ & $.297 \pm .017$ & $.252 \pm .017$ & $.585 \pm .014$ & $.662 \pm .015$ & $.586 \pm .017$ \\
        & $.1$ & $.348 \pm .019$ & $.196 \pm .015$ & $.216 \pm .018$ & $.642 \pm .015$ & $.662 \pm .014$ & $.535 \pm .016$ \\
        & $.01$ & $.321 \pm .018$ & $.251 \pm .020$ & $.201 \pm .018$ & $.655 \pm .013$ & $.433 \pm .016$ & $.493 \pm .017$ \\
        & $.001$ & $.323 \pm .018$ & $.203 \pm .016$ & $.235 \pm .018$ & $.613 \pm .013$ & $.520 \pm .016$ & $.378 \pm .018$ \\
        \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.306 \pm .021$ & $.301 \pm .021$ & $.259 \pm .019$ & $.646 \pm .015$ & $.621 \pm .016$ & $.656 \pm .017$ \\
        & $.1$ & $.307 \pm .020$ & $.256 \pm .019$ & $.207 \pm .015$ & $.714 \pm .014$ & $.676 \pm .015$ & $.490 \pm .022$ \\
        & $.01$ & $.293 \pm .019$ & $.231 \pm .017$ & $.205 \pm .014$ & $.722 \pm .014$ & $.654 \pm .017$ & $.573 \pm .026$ \\
        & $.001$ & $.295 \pm .019$ & $.205 \pm .015$ & $.215 \pm .015$ & $.771 \pm .012$ & $.737 \pm .015$ & $.637 \pm .021$ \\
    \bottomrule
    \end{tabularx}
    \label{tab:beat_vae_mnist_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. For each model, we report mean and standard error of the mean on the row signed as M, while we report the worst case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{0.62\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} 
         & M & $.629 \pm .014$ & $\bf .646 \pm .014$ & $.532 \pm .011$ \\
         & W & $.339$ & $.349$ & $.286$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} 
         & M & $\bf .657 \pm .016$ & $\bf .660 \pm .015$ & $\bf .658 \pm .016$ \\
         & W & $.242$ & $.302$ & $.264$\\
    \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{0.66\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & $\beta$ & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.571 \pm .012$ & $.612 \pm .013$ & $.604 \pm .013$ \\
         & $.1$ & $.574 \pm .013$ & $.618 \pm .013$ & $.620 \pm .013$ \\
         & $.01$ & $.599 \pm .014$ & $.614 \pm .013$ & $.593 \pm .012$ \\
         & $.001$ & $.556 \pm .011$ & $.622 \pm .013$ & $.629 \pm .013$ \\
         \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.643 \pm .015$ & $.652 \pm .014$ & $\bf .668 \pm .014$ \\
        & $.1$ & $.661 \pm .014$ & $\bf .664 \pm .014$ & $\bf .659 \pm .015$ \\ 
        & $.01$ & $\bf .666 \pm .014$ & $\bf .661 \pm .014$ & $\bf .661 \pm .015$ \\ 
        & $.001$ & $\bf .664 \pm .014$ & $\bf .662 \pm .014$ & $\bf .671 \pm .014$ \\ 
    \bottomrule
    \end{tabularx}
    \label{tab:beta_vae_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

% \begin{table*}[ht]
%     \begin{center}
%     \caption{MAYO dataset, Gaussian measurements, AE and VAE. Performance metric is SSIM (higer is better). The reward for the RL policy is computed based on the step-by-step reconstruction error.}
    
%     \begin{tabularx}{\linewidth}{llcc}
%     \toprule
%         & & \multicolumn{2}{c}{Gaussian} \\
%          %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
%          \cmidrule(lr){3-4}\\
%         Models & $\beta$ & 20 & 50\\
%         \midrule
%         AE-R & $---$ & $.470 \pm .008$ & $.554 \pm .010$ \\
%         \midrule
%         AE-E2E & $---$ & $.489 \pm .009$ & $.588 \pm .014$ \\
%         \midrule
%          \multirow{4}{*}{VAE-R} 
%          & $1$ & $.441 \pm .007$ & $.552 \pm .010$ \\
%          & $.1$ & $.483 \pm .009$ & $---$ \\
%          & $.01$ & $.431 \pm .008$ & $---$ \\
%          & $.001$ & $.478 \pm .009$ & $---$ \\
%          \midrule
                
%         \multirow{3}{*}{VAE-E2E} 
%         & $1$ & $.498 \pm .009$ & $.520 \pm .009$ \\
%         & $.1$ & $.492 \pm .007$ & $---$ \\
%         & $.01$ & $.501 \pm .008$ & $---$ \\
%         & $.001$ & $.492 \pm .007$ & $---$ \\
%     \bottomrule
%     \end{tabularx}
%     \end{center}
% \vspace{-5mm}
% \end{table*}

==> tables/mayo_cs.tex <==
\begin{table*}[!ht]
\caption{CS results on MAYO. The reported results corresponding to 200 measurements. By Converged Points, we refer to points that, for a given number of iterations, resulted in MSE (per pixel) lower than $1.e^{-2}$. Concerning the MSE, we reported the mean value $\pm 1 \sigma$. The MSE is computed across converged points only. We emphasize in bold, results from the best model.}

\label{tab:mayo_cs_results}
\begin{center}
\begin{tabularx}{\linewidth}{@{}lll|YY|YY|YY|YY@{}}
\toprule
&&\multirow{2}{*}{Prior} & \multicolumn{2}{c|}{50 iterations} & \multicolumn{2}{c|}{100 iterations} & \multicolumn{2}{c|}{150 iterations} & \multicolumn{2}{c}{200 iterations} \\
&&& MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ \\ \midrule

&\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{No rotation}}}
& Flow & 8.9 $\pm$ 0.9 & 28.2 & 8.1 $\pm$ 1.2 & 65.9 & 7.3 $\pm$ 1.3 & 79.7 & 6.8 $\pm$ 1.4  & 86.8  \\
&& Aug-Flow & N/A & 0.0 & 8.2 $\pm$ 1.2 & 40.1 & 7.4 $\pm$ 1.4 & 77.1 & 6.7 $\pm$ 1.4 & 83.4 \\
&& Conv-VAE & 7.9 $\pm$ 1.3 & 39.9 & 6.8 $\pm$ 1.6 & 76.2 & 6.2 $\pm$ 1.8 & \bf{89.6} & 5.9 $\pm$ 1.8  & \bf{95.5}  \\
&& Aug-VAE & 7.5 $\pm$ 1.3 & 51.7 & \bf{6.1 $\pm$ 1.6} & 75.7 & \bf{5.7 $\pm$ 1.7} & 83.8 & \bf{5.5 $\pm$ 1.6}  & 88.1  \\
&& Eq-VAE &  \bf{7.4 $\pm$ 1.4} & \bf{73.5} & 6.4 $\pm$ 1.4 & \bf{86.9} & 6.1 $\pm$ 1.5  & 89.2  & 6.0 $\pm$ 1.5  & 90.4  \\ \midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Unknown}}}
& \multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{rotation}}}
& Flow & 7.2 $\pm$ 1.4 & \bf{76.4} & \bf{5.8 $\pm$ 1.5} & 83.8 & \bf{5.2 $\pm$ 1.6} & 87.5 & \bf{5.0 $\pm$ 1.7} & \bf{93.3}  \\
&& Aug-Flow & N/A & 0.0 & 8.2 $\pm$ 1.1 & 49.9 & 6.9 $\pm$ 1.3 & 80.9 & 6.0 $\pm$ 1.3 & 84.3 \\
&& Conv-VAE & \bf{7.1 $\pm$ 1.7} & 55.3 & 5.9 $\pm$ 2.1 & 80.5 & 5.4 $\pm$ 2.1 & 88.2 & 5.0 $\pm$ 2.0  & 90.2 \\
&& Aug-VAE & 7.5 $\pm$ 1.5 & 59.3 & 5.9 $\pm$ 1.6 & 85.2 & 5.3 $\pm$ 1.5 & 89.1 & 5.1 $\pm$ 1.6  & 92.4  \\
&& Eq-VAE &  7.6 $\pm$ 1.4 & 70.3 & 6.6 $\pm$ 1.5 & \bf{87.5} & 6.1 $\pm$ 1.5 & \bf{91.3} & 6.0 $\pm$ 1.6 & 92.7  \\ \midrule
\bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/mnist_ae_final_reward.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{Results on the MNIST datset for both Gaussian and Radon measurements in SSIM (higer is better). The reward for the RL policy is computed based on the final reconstruction error.}
    
    \begin{tabularx}{\linewidth}{llcccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.51 \pm .02$ & $.64 \pm .01$ & $.73 \pm .01$ & $.58 \pm .02$ & $.69 \pm .01$ & $.77 \pm .01$ \\
         & \multirow{1}{*}{W}   & $-.03$ & $.06$ & $.13$ & $-.01$ & $.08$ & $.17$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.33 \pm .02$ & $.22 \pm .02$ & $.40 \pm .02$ & $---$ & $---$ & $---$ \\
         & \multirow{1}{*}{W}   & $-.12$ & $-.15$ & $-.12$ & $---$ & $---$ & $---$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & $.48 \pm .02$ & $.30 \pm .02$ & $.28 \pm .02$ & $---$ & $---$ & $---$ \\
         & \multirow{1}{*}{W}   & $-.08$ & $-.16$ & $-.14$ & $---$ & $---$ & $---$ \\
         \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_abl}
    \end{center}
\end{table*}

==> tables/mnist_results.tex <==

\begin{table*}[ht]
\caption{CS results on MNIST. We report results averaged over 1000 test points. By Converged Points, we refer to points that, for a given number of iterations, resulted in MSE (per pixel) lower than $1.e^{-2}$. We emphasize in bold, results from the best model.}

\label{tab:mnist_cs_results}
\begin{center}
% \begin{sc}
% \begin{tabular}{l|ccc|ccc|ccc}
\begin{tabularx}{\linewidth}{@{}lll|YYc|YYc|YYc@{}}
\toprule
&&\multirow{2}{*}{Prior} & \multicolumn{3}{c|}{50 measurements} & \multicolumn{3}{c|}{100 measurements} & \multicolumn{3}{c}{200 measurements} \\
&&& MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter$\downarrow$ &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter$\downarrow$ &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter $\downarrow$\\ \midrule
&\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{No rotation}}}
& Flow        & 45.4 & 100 & 59 & 19.2 & 100 & 39 & 10.2 & 100 & 38 \\
&& Cond. Flow & 22.6 & 100 & 35 & 10.1 & 100 & \textbf{22} & 5.8 & 100 & \textbf{22} \\
&& MLP-VAE    & 25.7 & 100 & 50 & 12.1 & 100 & 41 & 8.7 & 100 & 38\\
&& Conv-VAE   & 18.0 & 100 & 48 & 5.5  & 100 & 39 & 3.2 & 100 & 35\\
&& Eq-VAE     & \textbf{10.6} & 100 & \textbf{34} & \textbf{2.6}  & 100 & \textbf{22} & \textbf{2.1} & 100 & \textbf{22}\\ \midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Unknown}}}
& \multirow {5}{*}{\STAB{\rotatebox[origin=c]{90}{rotation}}}
& Flow        & 27.2 & 100 & 73 & 13.2 & 100 & 60 & 7.6  & 100 & 36 \\
&& Cond. Flow & 17.9 & 100 & 42 & 7.2  & 100 & 32 & 6.0  & 100 & 30 \\
&& MLP-VAE    & 25.9 & 100 & 48 & 16.4 & 100 & 40 & 11.7 & 100 & 34\\
&& Conv-VAE   & 17.5 & 100 & 51 & 7.0  & 100 & 39 & 4.2  & 100 & 32\\
&& Eq-VAE     & \textbf{11.8} & 100 & \textbf{33} & \textbf{4.2}  & 100 & \textbf{24} & \textbf{3.2}  & 100 & \textbf{23}\\
\bottomrule
\end{tabularx}
% \end{sc}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables/vae.tex <==
\begin{table}[ht]
    \begin{center}
    \caption{Results in SSIM (higher is better) on MNIST test dataset and different trajectory lengths (number on second row). SSIM is computed at the end of each acquisition trajectory, and we report mean and standard error of the mean. We also report the $\beta$ parameter on the second column. We highlight in bold the best performance for each configuration. Concerning the setting with 50 Gaussian measurements, the performance of the best VAE-E2E and VAE-R agree within the error.}
    \begin{tabularx}{\linewidth}{llcccccccc}
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{1}{*}{VAE-R} & \multirow{1}{*}{$\beta=1$}  & $.44 \pm .02$ & $\bm{.63 \pm 0.02}$ & $\bm{.70 \pm .01}$ & $.55 \pm .02$ & $.68 \pm .01$ & $.737 \pm .011$ \\
         %& \multirow{1}{*}{$\beta=0.1$}   & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$\\
         %& \multirow{1}{*}{$\beta=0.01$}   & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $.193 \pm .010$ \\
         \midrule
        \multirow{3}{*}{VAE-E2E} & \multirow{1}{*}{$\beta=1$}  & $.569 \pm .018$ & $.595 \pm .017$ & $.578 \pm .018$ & $.768 \pm .011$ & $.832 \pm .009$ & $.852 \pm .008$ \\
         & \multirow{1}{*}{$\beta=0.1$}   & $.591 \pm .017$ & $.584 \pm .018$ & $.586 \pm .018$ & $.811 \pm .009$ & $.841 \pm .008$ & $.846 \pm .009$\\
         & \multirow{1}{*}{$\beta=0.01$}   & \bm{$.610 \pm .017$} & $.626 \pm .017$ & $.606 \pm .019$ & \bm{$.821 \pm .009$} & \bm{$.848 \pm .008$} & \bm{$.851 \pm .008$} \\
         \midrule
    \end{tabularx}
    \label{tab:vae}
    \end{center}
\end{table}

==> tables_iclr/NewResults.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean on the row signed as M, while we report the worst
    case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    \small
    \begin{tabularx}{\linewidth}{llcccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.505 \pm .018$ & $.641 \pm .014$ & $.726 \pm .011$ & $.658 \pm .014$ & $.664 \pm .014$ & $.757 \pm .011$ \\
         & \multirow{1}{*}{W}   & $-.028$ & $.064$ & $.132$ & $.074$ & $-.036$ & $.100$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.325 \pm .021$ & $.217 \pm .018$ & $.232 \pm .016$ & $.680 \pm .013$ & $.456 \pm .019$ & $.365 \pm .017$ \\
         & \multirow{1}{*}{W}   & $-.117$ & $-.153$ & $-.119$ & $.079$ & $-.120$ & $-.111$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & $.475 \pm .021$ & $.296 \pm .021$ & $.283 \pm .021$ & $.824 \pm .009$ & $.781 \pm .014$ & $.739 \pm .015$ \\
         & \multirow{1}{*}{W}   & $-.078$ & $-.162$ & $-.144$ & $.205$ & $.057$ & $.010$ \\
         \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mnist_abl}
    \end{center}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \small
    \begin{tabularx}{\linewidth}{llcccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & $\beta$ & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.441 \pm .018$ & $.627 \pm .014$ & $.703 \pm .012$ & $.566 \pm .016$ & $.639 \pm .015$ & $.733 \pm .012$ \\
         & $.1$ & $.467 \pm .017$ & $.629 \pm .015$ & $.701 \pm .012$ & $.581 \pm .015$ & $.678 \pm .012$ & $.743 \pm .011$ \\
         & $.01$ & $.482 \pm .016$ & $.635 \pm .014$ & $.696 \pm .012$ & $.595 \pm .014$ & $.714 \pm .012$ & $.761 \pm .010$ \\
         & $.001$ & $.479 \pm .016$ & $.635 \pm .014$ & $.706 \pm .012$ & $.612 \pm .014$ & $.675 \pm .013$ & $.764 \pm .010$ \\
         \midrule
         
        \multirow{3}{*}{VAE-P} 
        & $1$ & $.335 \pm .019$ & $.297 \pm .017$ & $.252 \pm .017$ & $.585 \pm .014$ & $.662 \pm .015$ & $.586 \pm .017$ \\
        & $.1$ & $.348 \pm .019$ & $.196 \pm .015$ & $.216 \pm .018$ & $.642 \pm .015$ & $.662 \pm .014$ & $.535 \pm .016$ \\
        & $.01$ & $.321 \pm .018$ & $.251 \pm .020$ & $.201 \pm .018$ & $.655 \pm .013$ & $.433 \pm .016$ & $.493 \pm .017$ \\
        & $.001$ & $.323 \pm .018$ & $.203 \pm .016$ & $.235 \pm .018$ & $.613 \pm .013$ & $.520 \pm .016$ & $.378 \pm .018$ \\
        \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.306 \pm .021$ & $.301 \pm .021$ & $.259 \pm .019$ & $.646 \pm .015$ & $.621 \pm .016$ & $.656 \pm .017$ \\
        & $.1$ & $.307 \pm .020$ & $.256 \pm .019$ & $.207 \pm .015$ & $.714 \pm .014$ & $.676 \pm .015$ & $.490 \pm .022$ \\
        & $.01$ & $.293 \pm .019$ & $.231 \pm .017$ & $.205 \pm .014$ & $.722 \pm .014$ & $.654 \pm .017$ & $.573 \pm .026$ \\
        & $.001$ & $.295 \pm .019$ & $.205 \pm .015$ & $.215 \pm .015$ & $.771 \pm .012$ & $.737 \pm .015$ & $.637 \pm .021$ \\
    \bottomrule
    \end{tabularx}
    \label{tab:beat_vae_mnist_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. For each model, we report mean and standard error of the mean on the row signed as M, while we report the worst case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} 
         & M & $.629 \pm .014$ & $\bf .646 \pm .014$ & $.532 \pm .011$ \\
         & W & $.339$ & $.349$ & $.286$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} 
         & M & $\bf .657 \pm .016$ & $\bf .660 \pm .015$ & $\bf .658 \pm .016$ \\
         & W & $.242$ & $.302$ & $.264$\\
    \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & $\beta$ & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.571 \pm .012$ & $.612 \pm .013$ & $.604 \pm .013$ \\
         & $.1$ & $.574 \pm .013$ & $.618 \pm .013$ & $.620 \pm .013$ \\
         & $.01$ & $.599 \pm .014$ & $.614 \pm .013$ & $.593 \pm .012$ \\
         & $.001$ & $.556 \pm .011$ & $.622 \pm .013$ & $.629 \pm .013$ \\
         \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.643 \pm .015$ & $.652 \pm .014$ & $\bf .668 \pm .014$ \\
        & $.1$ & $.661 \pm .014$ & $\bf .664 \pm .014$ & $\bf .659 \pm .015$ \\ 
        & $.01$ & $\bf .666 \pm .014$ & $\bf .661 \pm .014$ & $\bf .661 \pm .015$ \\ 
        & $.001$ & $\bf .664 \pm .014$ & $\bf .662 \pm .014$ & $\bf .671 \pm .014$ \\ 
    \bottomrule
    \end{tabularx}
    \label{tab:beta_vae_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

% \begin{table*}[ht]
%     \begin{center}
%     \caption{MAYO dataset, Gaussian measurements, AE and VAE. Performance metric is SSIM (higer is better). The reward for the RL policy is computed based on the step-by-step reconstruction error.}
    
%     \begin{tabularx}{\linewidth}{llcc}
%     \toprule
%         & & \multicolumn{2}{c}{Gaussian} \\
%          %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
%          \cmidrule(lr){3-4}\\
%         Models & $\beta$ & 20 & 50\\
%         \midrule
%         AE-R & $---$ & $.470 \pm .008$ & $.554 \pm .010$ \\
%         \midrule
%         AE-E2E & $---$ & $.489 \pm .009$ & $.588 \pm .014$ \\
%         \midrule
%          \multirow{4}{*}{VAE-R} 
%          & $1$ & $.441 \pm .007$ & $.552 \pm .010$ \\
%          & $.1$ & $.483 \pm .009$ & $---$ \\
%          & $.01$ & $.431 \pm .008$ & $---$ \\
%          & $.001$ & $.478 \pm .009$ & $---$ \\
%          \midrule
                
%         \multirow{3}{*}{VAE-E2E} 
%         & $1$ & $.498 \pm .009$ & $.520 \pm .009$ \\
%         & $.1$ & $.492 \pm .007$ & $---$ \\
%         & $.01$ & $.501 \pm .008$ & $---$ \\
%         & $.001$ & $.492 \pm .007$ & $---$ \\
%     \bottomrule
%     \end{tabularx}
%     \end{center}
% \vspace{-5mm}
% \end{table*}

==> tables_iclr/mayo.tex <==
\begin{table}[ht]
    \begin{center}
    \caption{Results on the MAYO datset for both Gaussian and Radon measurements, for trajectory length respectively of 50 and 10. We report mean and standard error of the mean in SSIM on the test set. We highlight in bold the best performance for each configuration.}
    \begin{tabularx}{0.65\linewidth}{lcccc}
    \toprule
        & Gaussian & & Radon \\
         %\cmidrule(lr){2-3} %\cmidrule(lr){2-4}\\
        Models & 50 & & 10\\
        \midrule
         AE-R & $\bm{.575 \pm .008}$ & & $.444 \pm .009$\\
         \midrule
        AE-E2E & $.506 \pm .008$ & & $\bm{.623 \pm .012}$\\
        VAE-R ($\beta=1$) & $.521 \pm .008$ & & $.551 \pm .010$\\
        VAE-E2E ($\beta=1$) & $.413 \pm .012$ & & $.608 \pm .011$\\
         \bottomrule
    \end{tabularx}
    \label{tab:mayo}
    \end{center}
\vspace{-5mm}
\end{table}

==> tables_iclr/mayo_cs.tex <==
\begin{table*}[!ht]
\caption{CS results on MAYO. The reported results corresponding to 200 measurements. By Converged Points, we refer to points that, for a given number of iterations, resulted in MSE (per pixel) lower than $1.e^{-2}$. Concerning the MSE, we reported the mean value $\pm 1 \sigma$. The MSE is computed across converged points only. We emphasize in bold, results from the best model.}

\label{tab:mayo_cs_results}
\begin{center}
\begin{tabularx}{\linewidth}{@{}lll|YY|YY|YY|YY@{}}
\toprule
&&\multirow{2}{*}{Prior} & \multicolumn{2}{c|}{50 iterations} & \multicolumn{2}{c|}{100 iterations} & \multicolumn{2}{c|}{150 iterations} & \multicolumn{2}{c}{200 iterations} \\
&&& MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$  &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ \\ \midrule

&\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{No rotation}}}
& Flow & 8.9 $\pm$ 0.9 & 28.2 & 8.1 $\pm$ 1.2 & 65.9 & 7.3 $\pm$ 1.3 & 79.7 & 6.8 $\pm$ 1.4  & 86.8  \\
&& Aug-Flow & N/A & 0.0 & 8.2 $\pm$ 1.2 & 40.1 & 7.4 $\pm$ 1.4 & 77.1 & 6.7 $\pm$ 1.4 & 83.4 \\
&& Conv-VAE & 7.9 $\pm$ 1.3 & 39.9 & 6.8 $\pm$ 1.6 & 76.2 & 6.2 $\pm$ 1.8 & \bf{89.6} & 5.9 $\pm$ 1.8  & \bf{95.5}  \\
&& Aug-VAE & 7.5 $\pm$ 1.3 & 51.7 & \bf{6.1 $\pm$ 1.6} & 75.7 & \bf{5.7 $\pm$ 1.7} & 83.8 & \bf{5.5 $\pm$ 1.6}  & 88.1  \\
&& Eq-VAE &  \bf{7.4 $\pm$ 1.4} & \bf{73.5} & 6.4 $\pm$ 1.4 & \bf{86.9} & 6.1 $\pm$ 1.5  & 89.2  & 6.0 $\pm$ 1.5  & 90.4  \\ \midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Unknown}}}
& \multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{rotation}}}
& Flow & 7.2 $\pm$ 1.4 & \bf{76.4} & \bf{5.8 $\pm$ 1.5} & 83.8 & \bf{5.2 $\pm$ 1.6} & 87.5 & \bf{5.0 $\pm$ 1.7} & \bf{93.3}  \\
&& Aug-Flow & N/A & 0.0 & 8.2 $\pm$ 1.1 & 49.9 & 6.9 $\pm$ 1.3 & 80.9 & 6.0 $\pm$ 1.3 & 84.3 \\
&& Conv-VAE & \bf{7.1 $\pm$ 1.7} & 55.3 & 5.9 $\pm$ 2.1 & 80.5 & 5.4 $\pm$ 2.1 & 88.2 & 5.0 $\pm$ 2.0  & 90.2 \\
&& Aug-VAE & 7.5 $\pm$ 1.5 & 59.3 & 5.9 $\pm$ 1.6 & 85.2 & 5.3 $\pm$ 1.5 & 89.1 & 5.1 $\pm$ 1.6  & 92.4  \\
&& Eq-VAE &  7.6 $\pm$ 1.4 & 70.3 & 6.6 $\pm$ 1.5 & \bf{87.5} & 6.1 $\pm$ 1.5 & \bf{91.3} & 6.0 $\pm$ 1.6 & 92.7  \\ \midrule
\bottomrule
\end{tabularx}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables_iclr/mnist_ae_final_reward.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{Results on the MNIST datset for both Gaussian and Radon measurements in SSIM (higer is better). The reward for the RL policy is computed based on the final reconstruction error.}
    
    \begin{tabularx}{\linewidth}{llcccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.51 \pm .02$ & $.64 \pm .01$ & $.73 \pm .01$ & $.58 \pm .02$ & $.69 \pm .01$ & $.77 \pm .01$ \\
         & \multirow{1}{*}{W}   & $-.03$ & $.06$ & $.13$ & $-.01$ & $.08$ & $.17$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.33 \pm .02$ & $.22 \pm .02$ & $.40 \pm .02$ & $---$ & $---$ & $---$ \\
         & \multirow{1}{*}{W}   & $-.12$ & $-.15$ & $-.12$ & $---$ & $---$ & $---$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & $.48 \pm .02$ & $.30 \pm .02$ & $.28 \pm .02$ & $---$ & $---$ & $---$ \\
         & \multirow{1}{*}{W}   & $-.08$ & $-.16$ & $-.14$ & $---$ & $---$ & $---$ \\
         \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_abl}
    \end{center}
\end{table*}

==> tables_iclr/mnist_random_vs_adaptive.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{Results on the MNIST datset for both Gaussian and Radon measurements in SSIM (higer is better). The trajectory length of the experiment is reported on the second row. For each model, we report mean and standard error of the mean on on the row signed as M, while we report the worst case error on the row signed as W. All results are computed on the whole test set for one run. We highlight in bold the best performance for each configuration.}
    \small
    \begin{tabularx}{\linewidth}{llccccccc}
        \toprule
        & & \multicolumn{3}{c}{Gaussian} & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){7-9}\\
        Models & & 20 & 50 & 100 & & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.49 \pm .02$ & $\bm{.64 \pm .02}$ & \bm{$.73 \pm .01$} & & $.58 \pm .02$ & $.69 \pm .01$ & $.77 \pm .01$ \\
         & \multirow{1}{*}{W}   & $-.01$ & \bm{$.07$} & \bm{$.21$} & & $-.01$ & $.08$ & $.17$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.49 \pm .02$ & $.42 \pm .02$ & $.40 \pm .02$ & & $.66 \pm .01$ & $.47 \pm .02$ & $.43 \pm .02$ \\
         & \multirow{1}{*}{W}   & $-.12$ & $-.10$ & $-.12$ & & $.03$ & $-.10$ & $-.06$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & \bm{$.62 \pm .02$} & $.59 \pm .02$ & $.60 \pm .02$ & & \bm{$.83 \pm .01$} & \bm{$.84 \pm .01$} & \bm{$.85 \pm .01$} \\
         & \multirow{1}{*}{W}   & \bm{$.01$} & $-.05$ & $.02$ & &\bm{$.22$} & \bm{$.26$} & \bm{$.23$} \\
    \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_app}
    \end{center}
\end{table*}

==> tables_iclr/mnist_random_vs_adaptive_mainpaper.tex <==
\begin{table*}[ht]
    \caption{Results on the MNIST datset for both Gaussian and Radon measurements in SSIM (higer is better). The trajectory length of the experiment is reported on the second row. All results are computed on the whole test set for one run. We highlight in bold the best performance for each configuration.}
    \begin{center}
    \small
    \begin{tabularx}{0.92\linewidth}{lccccccccc}
    \toprule
        & \multicolumn{3}{c}{Gaussian} & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){2-4} \cmidrule(lr){6-8}\\
        Models & 20 & 50 & 100 & & 5 & 10 & 20\\
        \midrule
         \multirow{1}{*}{AE-R}  & $.49 \pm .02$ & $\bm{.64 \pm .02}$ & \bm{$.73 \pm .01$} & & $.58 \pm .02$ & $.69 \pm .01$ & $.77 \pm .01$ \\ \midrule
         \multirow{1}{*}{AE-P}  & $.49 \pm .02$ & $.42 \pm .02$ & $.40 \pm .02$ & & $.66 \pm .01$ & $.47 \pm .02$ & $.43 \pm .02$ \\
         \multirow{1}{*}{AE-E2E} & \bm{$.62 \pm .02$} & $.59 \pm .02$ & $.60 \pm .02$ & & \bm{$.83 \pm .01$} & \bm{$.84 \pm .01$} & \bm{$.85 \pm .01$} \\
    \bottomrule
    \end{tabularx}
    
    \label{tab:random_vs_e2e_mainpaper}
    \end{center}
\end{table*}

==> tables_iclr/mnist_results.tex <==

\begin{table*}[ht]
\caption{CS results on MNIST. We report results averaged over 1000 test points. By Converged Points, we refer to points that, for a given number of iterations, resulted in MSE (per pixel) lower than $1.e^{-2}$. We emphasize in bold, results from the best model.}

\label{tab:mnist_cs_results}
\begin{center}
% \begin{sc}
% \begin{tabular}{l|ccc|ccc|ccc}
\begin{tabularx}{\linewidth}{@{}lll|YYc|YYc|YYc@{}}
\toprule
&&\multirow{2}{*}{Prior} & \multicolumn{3}{c|}{50 measurements} & \multicolumn{3}{c|}{100 measurements} & \multicolumn{3}{c}{200 measurements} \\
&&& MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter$\downarrow$ &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter$\downarrow$ &  MSE ($1.e^{-3}$)$\downarrow$ & Converged Points (\%)$\uparrow$ & \# iter $\downarrow$\\ \midrule
&\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{No rotation}}}
& Flow        & 45.4 & 100 & 59 & 19.2 & 100 & 39 & 10.2 & 100 & 38 \\
&& Cond. Flow & 22.6 & 100 & 35 & 10.1 & 100 & \textbf{22} & 5.8 & 100 & \textbf{22} \\
&& MLP-VAE    & 25.7 & 100 & 50 & 12.1 & 100 & 41 & 8.7 & 100 & 38\\
&& Conv-VAE   & 18.0 & 100 & 48 & 5.5  & 100 & 39 & 3.2 & 100 & 35\\
&& Eq-VAE     & \textbf{10.6} & 100 & \textbf{34} & \textbf{2.6}  & 100 & \textbf{22} & \textbf{2.1} & 100 & \textbf{22}\\ \midrule
\multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Unknown}}}
& \multirow {5}{*}{\STAB{\rotatebox[origin=c]{90}{rotation}}}
& Flow        & 27.2 & 100 & 73 & 13.2 & 100 & 60 & 7.6  & 100 & 36 \\
&& Cond. Flow & 17.9 & 100 & 42 & 7.2  & 100 & 32 & 6.0  & 100 & 30 \\
&& MLP-VAE    & 25.9 & 100 & 48 & 16.4 & 100 & 40 & 11.7 & 100 & 34\\
&& Conv-VAE   & 17.5 & 100 & 51 & 7.0  & 100 & 39 & 4.2  & 100 & 32\\
&& Eq-VAE     & \textbf{11.8} & 100 & \textbf{33} & \textbf{4.2}  & 100 & \textbf{24} & \textbf{3.2}  & 100 & \textbf{23}\\
\bottomrule
\end{tabularx}
% \end{sc}
\end{center}
% \vskip -0.1in
\end{table*}

==> tables_iclr/new_res_1.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean on the row signed as M, while we report the worst
    case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    \small
    \begin{tabularx}{\linewidth}{llcccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} & \multirow{1}{*}{M}  & $.505 \pm .018$ & $.641 \pm .014$ & $.726 \pm .011$ & $.658 \pm .014$ & $.664 \pm .014$ & $.757 \pm .011$ \\
         & \multirow{1}{*}{W}   & $-.028$ & $.064$ & $.132$ & $.074$ & $-.036$ & $.100$ \\
         \midrule
        \multirow{2}{*}{AE-P} & \multirow{1}{*}{M}  & $.325 \pm .021$ & $.217 \pm .018$ & $.232 \pm .016$ & $.680 \pm .013$ & $.456 \pm .019$ & $.365 \pm .017$ \\
         & \multirow{1}{*}{W}   & $-.117$ & $-.153$ & $-.119$ & $.079$ & $-.120$ & $-.111$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} & \multirow{1}{*}{M}  & $.475 \pm .021$ & $.296 \pm .021$ & $.283 \pm .021$ & $.824 \pm .009$ & $.781 \pm .014$ & $.739 \pm .015$ \\
         & \multirow{1}{*}{W}   & $-.078$ & $-.162$ & $-.144$ & $.205$ & $.057$ & $.010$ \\
         \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mnist_abl}
    \end{center}
\end{table*}

==> tables_iclr/new_res_2.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MNIST dataset for both Gaussian and Radon measurements in SSIM (higer is
    better). The trajectory length of the experiment is reported on the second row. For each model, we
    report mean and standard error of the mean. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \footnotesize
    \begin{tabularx}{\linewidth}{llcccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & $\beta$ & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.441 \pm .018$ & $.627 \pm .014$ & $.703 \pm .012$ & $.566 \pm .016$ & $.639 \pm .015$ & $.733 \pm .012$ \\
         & $.1$ & $.467 \pm .017$ & $.629 \pm .015$ & $.701 \pm .012$ & $.581 \pm .015$ & $.678 \pm .012$ & $.743 \pm .011$ \\
         & $.01$ & $.482 \pm .016$ & $.635 \pm .014$ & $.696 \pm .012$ & $.595 \pm .014$ & $.714 \pm .012$ & $.761 \pm .010$ \\
         & $.001$ & $.479 \pm .016$ & $.635 \pm .014$ & $.706 \pm .012$ & $.612 \pm .014$ & $.675 \pm .013$ & $.764 \pm .010$ \\
         \midrule
         
        \multirow{3}{*}{VAE-P} 
        & $1$ & $.335 \pm .019$ & $.297 \pm .017$ & $.252 \pm .017$ & $.585 \pm .014$ & $.662 \pm .015$ & $.586 \pm .017$ \\
        & $.1$ & $.348 \pm .019$ & $.196 \pm .015$ & $.216 \pm .018$ & $.642 \pm .015$ & $.662 \pm .014$ & $.535 \pm .016$ \\
        & $.01$ & $.321 \pm .018$ & $.251 \pm .020$ & $.201 \pm .018$ & $.655 \pm .013$ & $.433 \pm .016$ & $.493 \pm .017$ \\
        & $.001$ & $.323 \pm .018$ & $.203 \pm .016$ & $.235 \pm .018$ & $.613 \pm .013$ & $.520 \pm .016$ & $.378 \pm .018$ \\
        \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.306 \pm .021$ & $.301 \pm .021$ & $.259 \pm .019$ & $.646 \pm .015$ & $.621 \pm .016$ & $.656 \pm .017$ \\
        & $.1$ & $.307 \pm .020$ & $.256 \pm .019$ & $.207 \pm .015$ & $.714 \pm .014$ & $.676 \pm .015$ & $.490 \pm .022$ \\
        & $.01$ & $.293 \pm .019$ & $.231 \pm .017$ & $.205 \pm .014$ & $.722 \pm .014$ & $.654 \pm .017$ & $.573 \pm .026$ \\
        & $.001$ & $.295 \pm .019$ & $.205 \pm .015$ & $.215 \pm .015$ & $.771 \pm .012$ & $.737 \pm .015$ & $.637 \pm .021$ \\
    \bottomrule
    \end{tabularx}
    \label{tab:beat_vae_mnist_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

==> tables_iclr/new_res_3.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. For each model, we report mean and standard error of the mean on the row signed as M, while we report the worst case error on the row signed as W. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{0.7\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & & 5 & 10 & 20\\
        \midrule
         \multirow{2}{*}{AE-R} 
         & M & $.629 \pm .014$ & $\bf .646 \pm .014$ & $.532 \pm .011$ \\
         & W & $.339$ & $.349$ & $.286$ \\
         \midrule
        \multirow{2}{*}{AE-E2E} 
         & M & $\bf .657 \pm .016$ & $\bf .660 \pm .015$ & $\bf .658 \pm .016$ \\
         & W & $.242$ & $.302$ & $.264$\\
    \bottomrule
    \end{tabularx}
    \label{tab:random_vs_e2e_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

==> tables_iclr/new_res_4.tex <==
\begin{table*}[!ht]
    \begin{center}
    \caption{Results on the MAYO dataset for Radon measurements. The trajectory length of the experiment is reported on the second row. We report mean and standard error of the mean in SSIM. The reward for the RL policy is computed based on the reconstruction error at the final state only.}
    
    \begin{tabularx}{0.8\linewidth}{llccc}
    \toprule
        & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5}\\
        Models & $\beta$ & 5 & 10 & 20\\
        \midrule
         \multirow{4}{*}{VAE-R} 
         & $1$ & $.571 \pm .012$ & $.612 \pm .013$ & $.604 \pm .013$ \\
         & $.1$ & $.574 \pm .013$ & $.618 \pm .013$ & $.620 \pm .013$ \\
         & $.01$ & $.599 \pm .014$ & $.614 \pm .013$ & $.593 \pm .012$ \\
         & $.001$ & $.556 \pm .011$ & $.622 \pm .013$ & $.629 \pm .013$ \\
         \midrule
         
        \multirow{3}{*}{VAE-E2E} 
        & $1$ & $.643 \pm .015$ & $.652 \pm .014$ & $\bf .668 \pm .014$ \\
        & $.1$ & $.661 \pm .014$ & $\bf .664 \pm .014$ & $\bf .659 \pm .015$ \\ 
        & $.01$ & $\bf .666 \pm .014$ & $\bf .661 \pm .014$ & $\bf .661 \pm .015$ \\ 
        & $.001$ & $\bf .664 \pm .014$ & $\bf .662 \pm .014$ & $\bf .671 \pm .014$ \\ 
    \bottomrule
    \end{tabularx}
    \label{tab:beta_vae_mayo_abl}
    \end{center}
\vspace{-5mm}
\end{table*}

==> tables_iclr/ppo.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{Comparison between PPO and VPG for different discount factors. All the models are trained with trajectories of 20 Gaussian acquisitions on the MNIST test dataset. We report mean and standard error of the mean at the end of the trajectory, in SSIM (higher is better). We highlight in bold the best performance across the different configurations.}
    
    \begin{tabularx}{0.8\linewidth}{lcccc}
    \toprule
        & \multicolumn{4}{c}{Gaussian - 20}\\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){2-5}\\
        Algorithm & $\gamma=0$ & $\gamma=0.9$ & $\gamma=0.99$ & $\gamma=1$\\
        \midrule
         \multirow{1}{*}{VPG} & $.577 \pm .017$ & $.616 \pm .017$ & $.634 \pm .016$ & $.618 \pm .017$ \\
         \midrule
        \multirow{1}{*}{PPO} & $.570 \pm .017$ & \bm{$.641 \pm .016$} & $.627 \pm .016$ & $.622 \pm .017$ \\
        \bottomrule
    \end{tabularx}
    \label{tab:ppo}
    \end{center}
\end{table*}

==> tables_iclr/vae.tex <==
\begin{table}[ht]
    \begin{center}
    \caption{Results in SSIM (higher is better) on MNIST test dataset and different trajectory lengths (number on second row). SSIM is computed at the end of each acquisition trajectory, and we report mean and standard error of the mean. We also report the $\beta$ parameter on the second column. We highlight in bold the best performance for each configuration. Concerning the setting with 50 Gaussian measurements, the performance of the best VAE-E2E and VAE-R agree within the error.}
    \begin{tabularx}{\linewidth}{llcccccccc}
        & & \multicolumn{3}{c}{Gaussian} & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){6-8}\\
        Models & & 20 & 50 & 100 & 5 & 10 & 20\\
        \midrule
         \multirow{1}{*}{VAE-R} & \multirow{1}{*}{$\beta=1$}  & $.44 \pm .02$ & $\bm{.63 \pm 0.02}$ & $\bm{.70 \pm .01}$ & $.55 \pm .02$ & $.68 \pm .01$ & $.737 \pm .011$ \\
         %& \multirow{1}{*}{$\beta=0.1$}   & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$\\
         %& \multirow{1}{*}{$\beta=0.01$}   & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $\mu \pm see$ & $.193 \pm .010$ \\
         \midrule
        \multirow{3}{*}{VAE-E2E} & \multirow{1}{*}{$\beta=1$}  & $.569 \pm .018$ & $.595 \pm .017$ & $.578 \pm .018$ & $.768 \pm .011$ & $.832 \pm .009$ & $.852 \pm .008$ \\
         & \multirow{1}{*}{$\beta=0.1$}   & $.591 \pm .017$ & $.584 \pm .018$ & $.586 \pm .018$ & $.811 \pm .009$ & $.841 \pm .008$ & $.846 \pm .009$\\
         & \multirow{1}{*}{$\beta=0.01$}   & \bm{$.610 \pm .017$} & $.626 \pm .017$ & $.606 \pm .019$ & \bm{$.821 \pm .009$} & \bm{$.848 \pm .008$} & \bm{$.851 \pm .008$} \\
         \midrule
    \end{tabularx}
    \label{tab:vae}
    \end{center}
\end{table}

==> tables_iclr/vae_mainpaper.tex <==
\begin{table}[ht]
    \begin{center}
    \caption{MNIST SSIM (the higher the better) for different trajectory lengths (number on second row). SSIM is computed at the end of each acquisition trajectory, and we report mean and standard error of the mean. We highlight in bold the best performance for each configuration. Note that for 50 Gaussian measurements, the performances of VAE-E2E and VAE-R agree within the error.}
    \small
    \begin{tabularx}{\linewidth}{llccccccccc}
    \toprule
        & & \multicolumn{3}{c}{Gaussian} & & \multicolumn{3}{c}{Radon} \\
         %& & \multicolumn{3}{c}{Nr. of latent dimensions} \\
         \cmidrule(lr){3-5} \cmidrule(lr){7-9}\\
        Models & $\beta$ & 20 & 50 & 100 & & 5 & 10 & 20\\
        \midrule
         \multirow{1}{*}{VAE-R} & \multirow{1}{*}{$1$}  & $.44 \pm .02$ & $\bm{.63 \pm 0.02}$ & $\bm{.70 \pm .01}$ & & $.55 \pm .02$ & $.68 \pm .013$ & $.74 \pm .01$ \\
         \midrule
         
        \multirow{3}{*}{VAE-E2E} & \multirow{1}{*}{$1$}  & $.57 \pm .02$ & $.60 \pm .02$ & $.58 \pm .02$ & & $.77 \pm .01$ & $.83 \pm .01$ & $.85 \pm .01$ \\
         & \multirow{1}{*}{$0.1$}   & $.59 \pm .02$ & $.58 \pm .02$ & $.59 \pm .02$ & & $.81 \pm .01$ & $.84 \pm .01$ & $.85 \pm .01$\\
         & \multirow{1}{*}{$0.01$}   & \bm{$.61 \pm .02$} & $.63 \pm .02$ & $.61 \pm .02$ & & \bm{$.82 \pm .01$} & \bm{$.85 \pm .01$} & \bm{$.85 \pm .01$} \\
         \bottomrule
    \end{tabularx}
    
    \label{tab:vae_mainpaper}
    \end{center}
\vspace{-5mm}
\end{table}
